Towards Federated Digital Twin Platforms

Digital Twin (DT) technology has become rather popular in recent years, promising to optimize production processes, manage the operation of cyber-physical systems, with an impact spanning across multiple application domains (e.g., manufacturing, robotics, space etc.). DTs can include different kinds of assets, e.g., models, data, which could potentially be reused across DT projects by multiple users, directly affecting development costs, as well as enabling collaboration and further development of these assets. To provide user support for these purposes, dedicated DT frameworks and platforms are required, that take into account user needs, providing the infrastructure and building blocks for DT development and management. In this demo paper, we show how the DT as a Service (DTaaS) platform has been extended to enable a federated approach to DT development and management, that allows multiple users across multiple instances of DTaaS to discover, reuse, reconfigure, and modify existing DT assets.

==> eptcsdata.tex <==
\providecommand{\firstpage}{32}
\providecommand{\publicationstatus}{M. Chechik et al. (Eds.): First International Workshop\\
on Autonomous Systems Quality Assurance and Prediction\\
with Digital Twins (ASQAP 2025)\\
EPTCS 418, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.418.4}{10.4204/EPTCS.418.4}}
\pdfoutput=1

